EtiCor: Corpus for Analyzing LLMs for Etiquettes

Etiquettes are an essential ingredient of day-to-day interactions among people. Moreover, etiquettes are region-specific, and etiquettes in one region might contradict those in other regions. In this paper, we propose EtiCor, an Etiquettes Corpus, having texts about social norms from five different regions across the globe. The corpus provides a test bed for evaluating LLMs for knowledge and understanding of region-specific etiquettes. Additionally, we propose the task of Etiquette Sensitivity. We experiment with state-of-the-art LLMs (Delphi, Falcon40B, and GPT-3.5). Initial results indicate that LLMs, mostly fail to understand etiquettes from regions from non-Western world.

==> sources.tex <==
\onecolumn  
\section{Corpus Sources} \label{app:corpus-source}
Websites used for scrapping Etiquettes for different regions are as follows:

\begin{itemize}
  \item
 {\textbf{Indian Culture: Do's and Don'ts}}\\ \url{https://culturalatlas.sbs.com.au/indian-culture/indian-culture-do-s-and-don-ts#indian-culture-do-s-and-don-ts}
  
  \item{ \textbf{Indian and Western Values}} \\ \url{https://www.studocu.com/in/document/sree-sankaracharya-university-of-sanskrit/social-work-in-education/indian-and-western-values/31773443}

  \item{\textbf{Which is the best culture: Indian or Western? (Quora)}}  \\ \url{https://www.quora.com/Which-is-the-best-culture-Indian-or-Western}

  
  \item {\textbf{Indian Culture: Etiquette}} \\ \url{https://culturalatlas.sbs.com.au/indian-culture/indian-culture-etiquette#indian-culture-etiquette}

  
  \item{\textbf{Indian Culture: Core Concepts}}  \\ \url{https://culturalatlas.sbs.com.au/indian-culture/indian-culture-core-concepts#indian-culture-core-concepts}
 
  
  \item {\textbf{Asian Customs and Values}} \\ \url{https://asiasociety.org/education/asian-customs-and-values}

  
  \item{\textbf{Indian Etiquette}}  \\ \url{https://www.a-to-z-of-manners-and-etiquette.com/indian-etiquette.html}
  
  \item {\textbf{Indian Culture: References}} \\ \url{https://culturalatlas.sbs.com.au/indian-culture/indian-culture-references#indian-culture-references}

  
  \item {\textbf{Indian People and Life}} \\ \url{https://factsanddetails.com/india/People_and_Life/sub7_3d/entry-4174.html}

  
  \item {\textbf{Difference Between Indian Culture and Western Culture (Ask Any Difference)}} \\ \url{https://askanydifference.com/difference-between-indian-culture-and-western-culture/}
  
  \item {\textbf{Indian Culture Compared to Japanese Culture}} \\ \url{https://smrutiprakashcom.wordpress.com/#:~:text=Indian%20culture%20compared%20to%20Japanese,culture%20primarily%20focuses%20on%20formality}

  
  \item{\textbf{Work Culture in Japan Compared to India (Quora)}}  \\ \url{https://www.quora.com/How-is-the-work-culture-in-Japan-in-comparison-to-India}
 
  
  \item {\textbf{Indians in Japan: Jugaad}} \\ \url{https://globisinsights.com/purpose/dei/indians-in-japan-jugaad/}
  
  \item{ \textbf{Japan v/s India: The Way Business is Run}}  \\ \url{https://blog.clrskills.com/japan-v-s-india-the-way-business-is-run/}

  
  \item{\textbf{Japan's Unique and Distinctive Work Culture}}  \\
\url{https://corporatecitizen.in/v6-Issue8/work-culture-japans-unique=and-distinctive-work-culture.html}
  
  \item{\textbf{Comparison Between Indian Work Culture and Japanese Work Culture}} \\
  \url{https://pdfcoffee.com/comparison-between-indian-work-culture-and-japanese-work-culture-with-regards-to-different-companies-pdf-free.html}
 
  \item{\textbf{India, Japanese Work Culture, and Mental Health}}  \\
\url{https://zeromindlab.com/india-japanese-work-culture-and-mental-health/}
  
  \item {\textbf{Japanese and Indian Work Cultures Are Starkly Different} }\\
  \url{https://economictimes.indiatimes.com/japanese-and-indian-work-cultures-are-starkly-different-geetanjali-kirloskar/articleshow/45977707.cms}
   
  \item {\textbf{5 Ways Japanese Work Culture is Drastically Different from the US}}\\\url{https://www.businessinsider.in/miscellaneous/5-ways-japanese-work-culture-is-drastically-different-from-the-us/slidelist/63523605.cms}

  \item{ \textbf{Similarities and Differences Between India and the Middle East (Quora)}\\ \url{https://www.quora.com/What-are-the-similarities-and-differences-between-India-and-the-Middle-East}} 

  \item \textbf{Differences Between Arabs and Indians} \\
  \url{http://www.differencebetween.net/miscellaneous/culture-miscellaneous/differences-between-arabs//-and-indians/}
  
  \item \textbf{Difference Between Arabs and Indians (Ask Any Difference)} 
  \url{https://askanydifference.com/difference-between-arabs-and-\\indians/}
  
  \item \textbf{India and the Middle East: Similarities in Cuisine} \\
  \url{https://en.vogue.me/culture/india-middle-east-cuisine-food-dishes-similarities/}
  
  \item \textbf{India and Africa: Similarities and Differences} \\
  \url{https://www.jstor.org/stable/40835868?searchText=&searchUri=&ab_segments=&searchKey=&refreqid=fastly-default%3A10c9bfae536e5ad2f656cebdc14b5c79&seq=5}

  \item \textbf{Cultural Diversity in India and Africa: A Strength, Not a Problem} \\
  \url{https://africaindia.org/cultural-diversity-in-india-and-africa-a-strength-not-a-problem/}
  
  \item \textbf{Japanese Culture: Do's and Don'ts} \\
\url{https://expertworldtravel.com/dos-donts-japanese-culture-tips/}

\item \textbf{Japanese Culture: Greetings} \\
\url{https://culturalatlas.sbs.com.au/japanese-culture/japanese-culture-greetings}

\item \textbf{Japanese Culture: Family} \\
\url{https://culturalatlas.sbs.com.au/japanese-culture/japanese-culture-family}

\item \textbf{Japanese Culture: Naming} \\
\url{https://culturalatlas.sbs.com.au/japanese-culture/japanese-culture-naming}

\item \textbf{Japanese Culture: Communication} \\
\url{https://culturalatlas.sbs.com.au/japanese-culture/japanese-culture-communication}

\item \textbf{Japanese Culture: Other Considerations} \\
\url{https://culturalatlas.sbs.com.au/japanese-culture/japanese-culture-other-\\considerations}

\item \textbf{Japanese Culture: Business Culture} \\
\url{https://culturalatlas.sbs.com.au/japanese-culture/japanese-culture-business-\\culture}

\item \textbf{Japanese Business Etiquette} \\
\url{https://planetdepos.com/trending/content/japanese-business-etiquette}

\item \textbf{Japan Guide: Etiquette and Customs} \\
\url{https://www.japan-guide.com/e/e622.html}

\item \textbf{South Korean Culture: Greetings} \\
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-greetings}

\item \textbf{South Korean Culture: Family} \\
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-family}

\item \textbf{South Korean Culture: Naming} \\
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-naming}

\item \textbf{South Korean Culture: Etiquette} \\
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-etiquette}

\item \textbf{South Korean Culture: Do's and Don'ts} \\
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-do-s-and-don-ts}

\item \textbf{South Korean Culture: Communication} \\
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-communication}

\item \textbf{South Korean Culture: Other Considerations} \\
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-other-considerations}

\item \textbf{South Korean Culture: Business Culture} \\
\url{https://culturalatlas.sbs.com.au/south-korean-culture/south-korean-culture-business-culture}

\item \textbf{Korean Etiquette} \\
\url{https://www.90daykorean.com/korean-etiquette/}

\item \textbf{Cramming Korean: Please Take Care of Me} \\
\url{https://noonasoverforks.com/2014/09/01/cramming-korean-please-take-care-of-me/}

\item \textbf{How to Greet People in Korea: 2 Steps with Pictures} \\
\url{https://medium.com/story-of-eggbun-education/how-to-greet-people-in-korea\\-2-steps-with-pictures-3cc4bd6d25c3}

\item \textbf{Taiwan Etiquette} \\
\url{http://www.ediplomat.com/np/cultural_etiquette/ce_tw.htm}

\item \textbf{Culture, Customs, and Etiquette in Taiwan} \\
\url{https://www.commisceo-global.com/resources/country-guides/taiwan-guide}

\item \textbf{Taiwanese Culture: Greetings} \\
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-greetings}

\item \textbf{Taiwanese Culture: Family} \\
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-family}

\item \textbf{Taiwanese Culture: Naming} \\
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-naming}

\item \textbf{Taiwanese Culture: Etiquette} \\
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-etiquette}

\item \textbf{Taiwanese Culture: Do's and Don'ts} \\
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-do-s-and-don-ts}

\item \textbf{Taiwanese Culture: Communication} \\
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-communication}

\item \textbf{Taiwanese Culture: Other Considerations} \\
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-other-considerations}

\item \textbf{Taiwanese Culture: Business Culture} \\
\url{https://culturalatlas.sbs.com.au/taiwanese-culture/taiwanese-culture-business-culture}
\item \textbf{Arab Academy: Your Guide to Arab Etiquette} \\
\url{https://www.arabacademy.com/your-guide-to-arab-etiquette/}

\item \textbf{Etiquette in the Middle East (Wikipedia)} \\
\url{https://en.m.wikipedia.org/wiki/Etiquette_in_the_Middle_East}

\item \textbf{Middle East Etiquette Tips} \\
\url{https://www.travelawaits.com/2494430/middle-east-etiquette/}

\item \textbf{Etiquette 101: The Do's and Don'ts of Visiting an Arab Home} \\
\url{https://theculturetrip.com/middle-east/united-arab-emirates/articles/etiquette-101-the-dos-and-donts-of-visiting-an-arab-home/}

\item \textbf{Arabic Customs and Etiquette: What to Consider When in the Middle East} \\
\url{https://kaleela.com/en/arabic-customs-and-etiquette-what-to-consider-when-in-middle-east}

\item \textbf{Manners in the Middle East (Aramco World)} \\
\url{https://archive.aramcoworld.com/issue/196502/manners.in.the.middle.east.html}

\item \textbf{South African Culture: Etiquette} \\
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-etiquette}

\item \textbf{South African Culture: Greetings} \\
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-greetings}

\item \textbf{South African Culture: Naming} \\
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-naming}

\item \textbf{South African Culture: Do's and Don'ts} \\
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-do-s-and-don-ts}

\item \textbf{South African Culture: Communication} \\
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-communication}

\item \textbf{South African Culture: Other Considerations} \\
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-other-considerations}

\item \textbf{South African Culture: Business Culture} \\
\url{https://culturalatlas.sbs.com.au/south-african-culture/south-african-culture-business-culture}

\item \textbf{Zimbabwean Culture: Greetings} \\
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-greetings}

\item \textbf{Zimbabwean Culture: Family} \\
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-family}

\item \textbf{Zimbabwean Culture: Naming} \\
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-naming}

\item \textbf{Zimbabwean Culture: Etiquette} \\
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-etiquette}

\item \textbf{Zimbabwean Culture: Do's and Don'ts} \\
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-do-s-and-don-ts}

\item \textbf{Zimbabwean Culture: Communication} \\
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-communication}

\item \textbf{Zimbabwean Culture: Other Considerations} \\
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-other-considerations}

\item \textbf{Zimbabwean Culture: Business Culture} \\
\url{https://culturalatlas.sbs.com.au/zimbabwean-culture/zimbabwean-culture-business-culture}

\item \textbf{Etiquette in Latin America (Wikipedia)} \\
\url{https://en.wikipedia.org/wiki/Etiquette_in_Latin_America}

\item \textbf{Business Etiquette in Latin America} \\
\url{https://www.jeffreygroup.com/agency-perspectives/business-etiquette-in-latin-america/}

\item \textbf{Cultural Pitfalls to Avoid in Latin America} \\
\url{https://www.allianceexperts.com/the-most-important-cultural-pitfalls-to-avoid-in-latin-america/}

\item \textbf{The Etiquette of Business in Latin America} \\
\url{https://www.languagereach.com/the-etiquette-of-business-in-latin-america/}

\item \textbf{South American Etiquette: How Different Is It?} \\
\url{https://thespanishgroup.org/blog/how-different-is-south-american-etiquette-from-the-rest-of-the-world/}

\end{itemize}
